Naturalness as a reasonable scientific principle in fundamental physics

I aim to clarify the physical content and significance of naturalness. Physicists' earliest understanding of naturalness, as an autonomy of scales (AoS) requirement provides the most cogent definition of naturalness and I will assert that i) this provides a uniform notion which undergirds a myriad prominent naturalness conditions, ii) this is a reasonable criterion to impose on EFTs and iii) the successes and violations of naturalness are best understood when adhering to this notion of naturalness. I argue that this principle is neither an aesthetic nor a sociologically-influenced principle. I contend that naturalness may only be plausibly argued to be an aesthetic/sociological principle when formal measures of naturalness and their use in physics communities are conflated with the central dogma of naturalness - the former may indeed be argued to be sociologically-influenced and somewhat arbitrary - but these formal measures of naturalness are in fact less successful than AoS naturalness. I put forward arguments as to why AoS naturalness is well-defined and why it was reasonable for physicists to endorse this naturalness principle on both theoretical and empirical grounds. Up to date, no compelling reasons have appeared as to why the laws of nature should generically decoupling into quasi-autonomous physical domains. A decoupling of scales in the quantum realm is often claimed to be entailed by the Decoupling Theorem (Cao and Schweber (1993)), yet I will show that this theorem is too weak to underwrite quasi-autonomous physical domains in quantum field theories because one should additionally impose that parameters be natural. Violations of naturalness would then have ontological import - unnatural parameters would not be accurately described by EFTs but rather by field theories exhibiting some kind of UV/IR interplay.

==> Extra.tex <==

\section*{Extra information}
\subsection*{The flatness problem (optional)}
Another troublesome fine-tuning problem (albeit not in the context of EFTs) is known to exist in cosmology and pertains to the curvature of spacetime.
The Friedmann equations are the equations in cosmology which govern the expansion of space within the context of general relativity, when homogeneneity and isotropy 
are assumed in models of the universe. The first Friedmann equation implies that the contribution from the curvature density must have been incredibly small in the early universe (as will now be discussed).
\nn
The first Friedmann equation can be written as follows
\begin{equation}\label{key}
\frac{8\pi}{3 M_p^2} \left[
{\rho_0^{\text{r}} \over (a \dot{a} )^2 } + {\rho_0^{\text{m}} \over a \dot{a}^2 } 
\right]
+ \frac{\Lambda}{3} \frac{a^2}{\dot{a}^2} - \frac{\kappa^2}{\dot{a}^2} = 1,
\end{equation}
where $a$ is a scale-factor (and $\dot{a}$ its time-derivative),  $\rho_0^{(\text{r,m})}$ denotes the density of radiation
and matter in the universe and $\kappa$ is the curvature parameter. Experimental data has unambiguously shown that the universe expands in an accelerating rate (implying $\dot{a}>0$). Since the scale-factor increases, the cosmological constant will dominate at ``late times'' in the universe entailing $\frac{\Lambda}{3} \frac{a^2}{\dot{a}^2} \simeq 1$. We should also note that the contributions from $\rho_0^{(\text{r,m})}$ increase significantly slower than the contribution from $\kappa^2$.
This brings about an interesting conclusion, because
the spatial curvature of our universe in the current cosmological epoch is positive, although the value is so low that the universe is approximately flat (described by $\kappa \approx 0$). The first Friedmann equation implies that the curvature must have been incredibly tiny in the early universe, where $\kappa = 10^{-60}$ is an often mentioned initial value in the literature.\footnote{The exact value depends on when (how much time after the big Bang) one sets the initial conditions. The flatness problem would still be problematic even if, say, $\kappa = 10^{-40}$ so we should not be bothered by the decimals of $\kappa$ - what is important is that $\kappa_0 \ll 1$.} This is intricately related to a fine-tuning problem - a minute variation of $\kappa_0'$ such as $\kappa_0 \rightarrow \kappa_0' = \kappa_0 + 10^{-20}$ would result in a universe whose spacetime would still be curved nowadays.


